In-IDE Code Generation from Natural Language: Promise and Challenges

A great part of software development involves conceptualizing or communicating the underlying procedures and logic that needs to be expressed in programs. One major difficulty of programming is turning concept into code, especially when dealing with the APIs of unfamiliar libraries. Recently, there has been a proliferation of machine learning methods for code generation and retrieval from natural language queries, but these have primarily been evaluated purely based on retrieval accuracy or overlap of generated code with developer-written code, and the actual effect of these methods on the developer workflow is surprisingly unattested. We perform the first comprehensive investigation of the promise and challenges of using such technology inside the IDE, asking "at the current state of technology does it improve developer productivity or accuracy, how does it affect the developer experience, and what are the remaining gaps and challenges?" We first develop a plugin for the IDE that implements a hybrid of code generation and code retrieval functionality, and orchestrate virtual environments to enable collection of many user events. We ask developers with various backgrounds to complete 14 Python programming tasks ranging from basic file manipulation to machine learning or data visualization, with or without the help of the plugin. While qualitative surveys of developer experience are largely positive, quantitative results with regards to increased productivity, code quality, or program correctness are inconclusive. Analysis identifies several pain points that could improve the effectiveness of future machine learning based code generation/retrieval developer assistants, and demonstrates when developers prefer code generation over code retrieval and vice versa. We release all data and software to pave the road for future empirical studies and development of better models.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> discussion_points.tex <==


% With the recent advancements in neural networks and deep learning in natural language 
% processing, there are multiple examples of systems attempting to generate 
% arbitrary code in a general-purpose programming language given natural language 
% inputs~\cite{yin2017syntactic,yin2018tranx,Iyer2018MappingLT,Agashe2019JuICeAL}.
% For example, \citet{yin2018tranx} proposed a syntactic tree-based neural 
% network model that encodes natural language utterances and generates abstract 
% syntax trees of the target code snippets; when instantiated for Python,
% the system can generate short code snippets given English descriptions of
% intent, \eg the code snippet ``\texttt{x.sort(reverse=True)}'' given the
% natural language input ``sort list \texttt{x} in reverse order''.
% Similarly, \citet{Iyer2018MappingLT} proposed a system to generate class 
% member functions given natural language descriptions of intent and the 
% programmatic context provided by the rest of the class.
% Finally, \citet{Agashe2019JuICeAL} proposed a system to generate the API 
% call sequence in a Jupyter Notebook code cell given the natural language 
% and code history up to that particular cell.
% We are still a ways away from not having to write any code while programming, 
% but all these systems reportedly have reasonable accuracy on benchmark datasets, 
% which makes our research study of their practical usefulness timely.

%=====================DISCUSSION=====================
% Looking at the percentage of the ``good queries'', we find that one outstanding barrier for deploying such code generation systems into real world development is that the user are not very often issue good queries that contain enough information even for a human programmer to implement the query intent.
% It is also the case that users sometime ignore to include key information inside the code context, like variables, etc. to inform the code generation model.
% This lead to potential gains in code generation model performance by incorporating more contextual information with natural language queries as input.
%======================================================


%====================DISCUSSION===================
% These suggest that code retrieval is more suitable for longer code snippets that have more complex functionalities packed together in the implementation, while code generation is suitable for shorter code snippets with simpler functionalities whose intent could be described sufficiently in the natural language query.
% Similar observations have also been indirectly found in previous analysis.
% We may use code retrieval to find relevant code that requires some editing to adapt to the current context, even with a few keywords specifying the vague intent or functionality, but for code generation models, those under-specified natural language intent rarely produces good results.
% However, for those simpler and shorter functionalities, code generation may have a better chance to generate better code snippets that take the details such as variable names or arguments specified in the query into account.
% Both code generation and code retrieval should be useful in such a real-world programming assistant plugin.
%====================================================
\
%====================DISCUSSION=====================
% \begin{quote}
% ``the plugin excels in letting you look up little syntax bits that you have forgotten, but where you have a good background understanding of the underlying principles/modules/frameworks.'' \partic{11}
% \end{quote}
%===================================================

%%%%%%%%%%%%%%%%%%%DISCUSSION
% These functionalities are basic but crucial in a wide variety of applications, and the fact that study participants prefer to use snippets produced by the code generation model here indicates that code generation provides effective suggestions for these sorts of simple queries.
% This is an intuitive result, as the code retrieval model could find relevant code snippets, often quite long and complete, given only a few keywords describing the intent.

% we expect that the users are more likely to use the code retrieval for the single query that contains complex intents that would usually requires multiple steps and sub-queries to fulfill, because this way the user would get more ``free code'' from the longer retrieved snippets.
% Besides, if users are familiar with using web search engines to search for programming questions, their queries may be more suited to a code retrieval approach (which requires less specified queries) than a generation approach (which requires more specified queries)

% Another interesting discovery is that the term ``python'' is also one of the highest weighted features for those end up using code retrieval. 
% Our reasoning is that the users have the habit of using web search engines to search for programming questions and help, so that they tend to always include ``python'' as a specifying keyword in those queries, even though this is not required in this particular code retrieval scenario.
% The results seen from the analysis are in line with our hypothesis in this section on the expected relative benefits of code retrieval and code generation.

% we find that both code generation and code retrieval could help different aspects of queries and intents in real use scenarios, and thus future research and development of both types of models would be valuable.
%%%%%%%%%%%%%%%%%%%



==> lmer_code_complexity.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Wed, Dec 30, 2020 - 22:18:37
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Code Complexity} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-2} D{.}{.}{-2} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{Code Complexity (cyclomatic complexity)} \\ 
 & \multicolumn{1}{c}{LME (default)} & \multicolumn{1}{c}{LME (de-meaned)} \\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)}\\ 
\hline \\[-1.8ex] 
 Experience & -0.21 &  \\ 
  & (0.46) &  \\ 
  Experience BTW &  & 0.04 \\ 
  &  & (0.74) \\ 
  Experience WI &  & -0.35 \\ 
  &  & (0.56) \\ 
  Uses plugin & 0.73 & 0.74 \\ 
  & (0.58) & (0.58) \\ 
  Constant & 5.64^{***} & 4.62 \\ 
  & (1.95) & (3.07) \\ 
 \hline \\[-1.8ex] 
Observations & 237 & 237 \\ 
Num users & 31 & 31 \\ 
Num tasks & 14 & 14 \\ 
sd(user) & 1.183 & 1.172 \\ 
sd(task) & 2.329 & 2.321 \\ 
R2m & 0.006 & 0.007 \\ 
R2c & 0.27 & 0.269 \\ 
Akaike Inf. Crit. & \multicolumn{1}{c}{1,417.27} & \multicolumn{1}{c}{1,419.09} \\ 
Bayesian Inf. Crit. & \multicolumn{1}{c}{1,438.08} & \multicolumn{1}{c}{1,443.36} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> lmer_program_correctness.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Dec 31, 2020 - 11:23:08
% Requires LaTeX packages: dcolumn 
\begin{table}[t] \centering 
  \caption{Program Correctness} 
  \label{tbl:program-correctness} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-2} D{.}{.}{-2} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{Program Correctness (score 0-10)} \\ 
 & \multicolumn{1}{c}{LME (default)} & \multicolumn{1}{c}{LME (de-meaned)} \\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)}\\ 
\hline \\[-1.8ex] 
 Experience & 0.02 &  \\ 
  & (0.22) &  \\ 
  Experience BTW &  & -0.17 \\ 
  &  & (0.37) \\ 
  Experience WI &  & 0.12 \\ 
  &  & (0.26) \\ 
  Uses plugin & 0.42 & 0.43 \\ 
  & (0.28) & (0.28) \\ 
  Constant & 6.11^{***} & 6.87^{***} \\ 
  & (0.95) & (1.52) \\ 
 \hline \\[-1.8ex] 
Observations & 264 & 264 \\ 
Num users & 35 & 35 \\ 
Num tasks & 14 & 14 \\ 
sd(user) & 0.78 & 0.77 \\ 
sd(task) & 1.19 & 1.17 \\ 
R2m & 0.007 & 0.009 \\ 
R2c & 0.303 & 0.3 \\ 
Akaike Inf. Crit. & \multicolumn{1}{c}{1,217.69} & \multicolumn{1}{c}{1,219.28} \\ 
Bayesian Inf. Crit. & \multicolumn{1}{c}{1,239.15} & \multicolumn{1}{c}{1,244.31} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> lmer_task_completion.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Dec 31, 2020 - 10:10:07
% Requires LaTeX packages: dcolumn 
\begin{table}[t] \centering 
  \caption{Task Completion Time} 
  \label{tbl:task-completion} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-2} D{.}{.}{-2} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{Task Completion Time (seconds)} \\ 
 & \multicolumn{1}{c}{LME (default)} & \multicolumn{1}{c}{LME (de-meaned)} \\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)}\\ 
\hline \\[-1.8ex] 
 Experience & -184.94 &  \\ 
  & (166.24) &  \\ 
  Experience BTW &  & -409.89 \\ 
  &  & (466.99) \\ 
  Experience WI &  & -156.03 \\ 
  &  & (175.36) \\ 
  Uses plugin & 102.36 & 101.93 \\ 
  & (178.31) & (178.28) \\ 
  Constant & 3,978.50^{***} & 4,901.58^{**} \\ 
  & (773.66) & (1,950.37) \\ 
 \hline \\[-1.8ex] 
Observations & 258 & 258 \\ 
Num users & 36 & 36 \\ 
Num tasks & 14 & 14 \\ 
sd(user) & 1429.56 & 1423.98 \\ 
sd(task) & 1136 & 1138.74 \\ 
R2m & 0.005 & 0.011 \\ 
R2c & 0.642 & 0.644 \\ 
Akaike Inf. Crit. & \multicolumn{1}{c}{4,579.06} & \multicolumn{1}{c}{4,580.80} \\ 
Bayesian Inf. Crit. & \multicolumn{1}{c}{4,600.38} & \multicolumn{1}{c}{4,605.67} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> lmer_task_performance_all_backup.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Jan 08, 2021 - 11:17:40
% Requires LaTeX packages: dcolumn 
\begin{table}[t] \centering 
  \caption{LMER task performance models (default specification).} 
  \label{tbl:task-performance} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-2} D{.}{.}{-2} D{.}{.}{-2} D{.}{.}{-2} } 
\\[-1.8ex]\toprule
\\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & \multicolumn{1}{c}{Completion time} & \multicolumn{1}{c}{Correctness score} & \multicolumn{1}{c}{SLOC} & \multicolumn{1}{c}{CC} \\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)}\\ 
\midrule \\[-1.8ex] 
 Experience & -195.62 & 0.07 & -0.62 & -0.21 \\ 
  & (183.11) & (0.24) & (1.61) & (0.46) \\ 
  Uses plugin & 15.76 & 0.44 & 4.16^{**} & 0.73 \\ 
  & (196.11) & (0.30) & (1.91) & (0.58) \\ 
  Constant & 3,984.51^{***} & 5.88^{***} & 27.15^{***} & 5.64^{***} \\ 
  & (838.07) & (1.03) & (7.40) & (1.95) \\ 
 \midrule \\[-1.8ex] 
Observations & 224 & 237 & 237 & 237 \\ 
Num users & 31 & 31 & 31 & 31 \\ 
Num tasks & 14 & 14 & 14 & 14 \\ 
sd(user) & 1489.25 & 0.82 & 6.16 & 1.18 \\ 
sd(task) & 1104.7 & 1.14 & 12.65 & 2.33 \\ 
R2m & 0.004 & 0.008 & 0.011 & 0.006 \\ 
R2c & 0.642 & 0.289 & 0.502 & 0.27 \\ 
Akaike Inf. Crit. & \multicolumn{1}{c}{3,987.14} & \multicolumn{1}{c}{1,106.66} & \multicolumn{1}{c}{2,002.42} & \multicolumn{1}{c}{1,417.27} \\ 
Bayesian Inf. Crit. & \multicolumn{1}{c}{4,007.61} & \multicolumn{1}{c}{1,127.46} & \multicolumn{1}{c}{2,023.23} & \multicolumn{1}{c}{1,438.08} \\ 
\bottomrule \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> misc.tex <==
\section{Background}
\label{sec:background}

% \gn{What about other non-natural-language based low-code and no-code platforms? e.g. methods that allow the developers to express their intents in other ways such as sketching interface components, etc.}

Traditionally, programming has been performed by software developers who write code directly in programming languages for the majority of functionality they wish to implement.
However, acquiring the requisite knowledge to perform this task requires time-consuming training and practice, and even for skilled programmers, writing programs requires a great amount of time and effort.
To this end, there have been many recent developments on no-code or low-code software development platforms that allow both programmers and non-programmers to develop in modalities of interaction other than code~\cite{Sahay2020SupportingTU}.
Some examples include visual programming languages such as Scratch~\cite{Maloney2010TheSP} that offers a building-block style graphical user interface to implement logic.
In specific domains such as user interface design and prototyping, recent advances in deep learning models also enable developers to sketch the user interface visually and then automatically generates user interface code with the sketch~\cite{Beltramelli2018pix2codeGC}, or using existing screenshots~\cite{Nguyen2015ReverseEM}.

Besides visual no-code or low-code programming interfaces, there has also been much progress on program synthesis~\cite{Basin2004SynthesisOP,Feser2015SynthesizingDS,Feng2018ProgramSU,Bodk2008ProgramSB}, which uses input-output examples, logic sketches, etc. to automatically generate functions, with some recent advances that use machine learning models~\cite{Balog2017DeepCoderLT,Chen2019ExecutionGuidedNP,Ellis2019WriteEA,Shin2019ProgramSA}. 
Some work also generate programs from easier-to-write pseudo-code~\cite{Kulal2019SPoCSP,Zhong2020SemanticSF}.

\looseness=-1
In this paper, we focus on another interaction modality: using natural 
language to help developers write code.
% Given a natural language query carrying the intent of a desired step in a 
% program, there are two main classes of methods to obtain code implementing 
% this intent: 
% On the one hand, \emph{code retrieval} techniques aim to search for and 
% retrieve an existing code fragment in a code base; given the abundance of 
% code snippets on platforms such as Stack Overflow, it is plausible that a 
% lot of the code that one might write, especially for lower level functionality 
% and API usage primitives, already exists somewhere, therefore the main 
% challenge is search.
% On the other hand, \emph{code generation} techniques aim to synthesize 
% code fragments given (natural language) specifications, which is more 
% ambitious, but can be particularly useful if those exact target code 
% fragments do not exist anywhere yet.
% We discuss each of these in more detail next, followed by \bv{something}

% \emph{natural language to code generation} and \emph{natural language code retrieval}.

\subsection{NL2Code Generation}
% Recently a large number of tasks related to natural language and programming language have caught interests of researchers.
% We are particularly interested in code generation's potential of helping developers program with little or no programming required.
% This field is studied by many researchers from different aspects.

Code generation from natural language has been around for many years. 
Researchers have proposed that natural language dialogue could be a 
new form of human-computer interaction since nearly the 
advent of modern computers~\cite{heidorn1976automatic,Ginsparg1978NaturalLP,dijkstra1979foolishness,mihalcea2006nlp}.
The bulk of prior work either targeted domain-specific languages (DSLs),
or focused on task-specific code generation for general-purpose languages, 
where more progress could be made given the relatively constrained vocabulary 
and output code space.
Examples include generating formatted input file parsers~\cite{Lei2013FromNL}; 
structured, idiomatic sequences of API calls~\cite{Raghothaman2016SWIMSW}; 
regular expressions~\cite{Kushman2013UsingSU,Manshadi2013IntegratingPB,Parisotto2017NeuroSymbolicPS}; 
string manipulation DSL programs~\cite{Raza2015CompositionalPS}; 
card implementations for trading card games~\cite{DBLP:conf/acl/LingBGHKWS16};
and solutions to the simplest of programming competition-style problems~\cite{Balog2017DeepCoderLT}.

% Special purpose natural language to code generation has been explored, like generating from natural language specifications to program input parsers~\cite{Lei2013FromNL}, or synthesizing idiomatic snippets~\cite{Raghothaman2016SWIMSW}.
% Generating arbitrary code in a general-purpose language is a more challenging
% task, that was difficult to tackle with rule-based or symbolic machine 
% learning machinery, and hence much work on code generation was limited to 
% generating code for domain-specific languages (DSLs), \eg regular expressions~\cite{Kushman2013UsingSU,Manshadi2013IntegratingPB,Parisotto2017NeuroSymbolicPS}, string manipulation~\cite{Raza2015CompositionalPS}, 
% trading card games~\cite{DBLP:conf/acl/LingBGHKWS16},
% and the simplest of programming competition-style problems~\cite{Balog2017DeepCoderLT}.

% Natural language to code generation \emph{generates program snippets from natural language (NL)}.
% For example, if the input is ``sort list \texttt{x} in reverse order'', then the system would ideally output ``\texttt{x.sort(reverse=True)}'' in Python.

Generating arbitrary code in a general-purpose language is more challenging
and it is difficult to achieve with rule-based or symbolic machine learning machinery.
However, with the recent boom of neural networks and deep learning in 
natural language processing, such tasks are becoming more feasible. 
We are still a ways away from not having to write any code while programming,
but we can begin to expect help with small but relatively unconstrained tasks.
For example, given the natural language input ``sort list \texttt{x} in reverse order'', 
one can expect based on current technology~\cite{yin2017syntactic,yin2018tranx} 
the Python output ``\texttt{x.sort(reverse=True)}'' to be automatically generated.

These systems are quite sophisticated, involving a syntactic tree-based neural 
network model that encodes natural language utterances and generates abstract 
syntax trees of the target code snippets; they have been trained on both official 
API documentation and Stack Overflow questions and answers~\cite{xu2020incorporating}; 
and they can generate reasonable code fragments given short text inputs, as 
shown in Table~\ref{tab:case}.
Note how such models can generate syntactically correct code snippets by
construction; demonstrate ability to identify and incorporate a wide variety 
of API calls; and also have the ability to copy important information like 
string literals and variable names from the input natural language intent.

There are also similar systems%
\footnote{This is, of course, among the many other use cases for neural network models of code and natural language such as code summarization~\cite{Iyer2016SummarizingSC,Yao2018StaQCAS}, or embedding models that represent programming languages together with natural languages~\cite{Feng2020CodeBERTAP}. \citet{allamanis2018survey} provide a comprehensive survey of the use cases of machine learning models in this area.}
able to generate class member functions 
given natural language descriptions of intent and the programmatic 
context provided by the rest of the class~\cite{Iyer2018MappingLT},
and to generate the API call sequence in a Jupyter Notebook code cell
given the natural language and code history up to that particular  
cell~\cite{Agashe2019JuICeAL}.
Even though these systems focus on slightly different tasks, they are 
conceptually similar to the aforementioned approach by \citet{yin2018tranx}
in their design (comparable neural network architectures) and they achieve 
comparable levels of accuracy. \bv{Is this true?}
We choose to use the \citet{yin2018tranx} approach in our human study as one element 
of our NL2Code plugin because of our familiarity with the implementation
and the natural complementarity with code retrieval, discussed below.
% models as one element of our interface, along with code retrieval, below.


% generating class member functions given English documentation and the programmatic context provided by the rest of the class.  -- Iyer2018MappingLT

% To study code generation conditioned on a long context his- tory, we present JuICe, a corpus of 1.5 mil- lion examples with a curated test set of 3.7K instances based on online programming as- signments. Compared with existing contextual code generation datasets, JuICe provides re- fined human-curated data, open-domain code, and an order of magnitude more training data. Using JuICe, we train models for two tasks: (1) generation of the API call sequence in a code cell, and (2) full code cell generation, both conditioned on the NL-Code history up to a particular code cell. Experiments using current baseline code generation models show that both context and distant supervision aid in generation, and that the dataset is challenging for current systems. -- Agashe2019JuICeAL

% and and general-purpose natural language to code generation, like the example mentioned above with Python, is now closer to being within reach~\cite{DBLP:conf/acl/LingBGHKWS16,yin2017syntactic,Iyer2018MappingLT,Agashe2019JuICeAL}.%
% \footnote{This is, of course, among the many other use cases for neural network models of code and natural language such as code summarization~\cite{Iyer2016SummarizingSC,Yao2018StaQCAS}, or embedding models that represent programming languages together with natural languages~\cite{Feng2020CodeBERTAP}. \citet{allamanis2018survey} provide a comprehensive survey of the use cases of machine learning models in this area.}
% Due to the improvements of deep neural architectures and the data-driven nature of those methods, many new models have emerged with stronger performance with more training data.
% For instance, a syntax tree-based neural network model that encodes natural language utterances and generates abstract syntax trees of the target code snippets \cite{yin2017syntactic,yin2018tranx} trained on resources like API documentation and Stack Overflow questions and answers \cite{xu2020incorporating} can now generate reasonable code suggestions for shorter text snippets, as shown in Table~\ref{tab:case}.
% As is evident from the examples, such models can generate syntactically correct code snippets, demonstrate ability to identify and retrieve a wide variety of API calls, and also have the ability to copy important information like string literals and variable names from the natural language intent.
% We will use such models as one element of our interface, along with code retrieval, below.

\begin{table}[t]
\begin{center}
\begin{tabular}{l@{\tightcol}p{12cm}}
\toprule
% \multicolumn{2}{l}{Convert tuple \textit{t} to list.} \\
% \refmark & \inlineCode+list(t)+  \\
% \xmark & \inlineCode+b=list(zip(*t))+  \\
% \cmark & \inlineCode+t=list(t)+  \\
% \midrule
\multicolumn{2}{l}{Open a file ``\texttt{f.txt}'' in write mode.} \\
\refmark & \inlineCode+f = open('f.txt', 'w')+  \\
\cmark & \inlineCode+f = open('f.txt', 'w')+  \\
\midrule
\multicolumn{2}{l}{Read a csv file ``\texttt{data.csv}'' to dataframe.} \\
\refmark & \inlineCode+df = pd.read_csv('data.csv')+  \\
\cmark & \inlineCode+df = pd.read_csv('data.csv')+  \\
\midrule
\multicolumn{2}{p{12cm}}{Lower a string \textit{text} and remove non-alphanumeric characters aside from space.} \\
\refmark & \inlineCode+re.sub(r'[^\sa-zA-Z0-9]', '', text).lower().strip()+ \\
\cmark & \inlineCode+re.sub(r'[^\sa-zA-Z0-9]', '', text)+ \\
\midrule
\multicolumn{2}{p{12cm}}{Choose a random file from the directory contents of the C drive, `C:\textbackslash\textbackslash'.} \\
\refmark & \inlineCode+random.choice(os.listdir('C:\\'))+ \\
\cmark & \inlineCode+random.choice(os.path.expanduser('C:\\'))+\\
\bottomrule
\end{tabular}
\end{center}
\caption{Examples, where
\refmark is the ground-truth code snippet, and \cmark is the output from the state-of-the-art code generation model.
Correct and erroneous function calls are marked in {\color{deepblue}blue} and {\color{deepred}red} respectively.
\bv{It's not obvious that these are good examples because it seems that a retrieval model might return the same results. Can you pick some where generation does better than retrieval?}
}
\label{tab:case}
\end{table}

\subsection{NL2Code Retrieval}

In contrast to code generation, code retrieval, in our context, is to search for code snippets that are related to the given natural language query.
It is a cross-domain information retrieval problem that uses natural language to query large databases of existing source code.
The simplest way to do so is to start with existing information retrieval models designed for natural language search, and adapt then specifically for the source code domain through query reformulation or other methods~\cite{Haiduc2013AutomaticQR,Hill2014NLbasedQR,Keivanloo2014SpottingWC,Wei2015BuildingBD,Lu2015QueryEV,Vinayakarao2017ANNEIS}.
Other research work utilize deep learning models \cite{Allamanis2015BimodalMO,Iyer2016SummarizingSC,gu2018deep,husain2019codesearchnet} to train a relevance model between natural language queries and corresponding code snippets.
It is also possible to exploit code annotations to generate additional information to help improve code retrieval performance \cite{Yao2019CoaCorCA} or extracted abstract programming patterns and associated natural language keywords for more content-based code search~\cite{Keivanloo2014SpottingWC}.
Many of the models achieve good performance on human annotated relevance benchmark datasets between natural language and code snippets.

% One of the important features to bridge the semantics between natural language with the code is the documentation or ``docstring'' of the function or method.
% However it would only be beneficial for real development use to deploy such retrieval models in large scale, with code snippet candidates from virtually all repositories on the Internet.

Practically, however, many developers simply rely on generic natural-language search engines like Google to find appropriate code snippets by first locating pages that contain code snippets through natural language queries~\cite{sadowski2015developers} on programming QA websites like Stack Overflow.
In this paper, to emulate this, we integrate the behavior of opening the web browser and searching with web search engines for code snippet inside our plugin.
Our plugin queries the search engine directly from the IDE and then select top answers from Stack Overflow and extract the code snippets by heuristics.

Notably, code retrieval and code generation methods each have their own advantages.
As long as the quality of the retrieval database can be appropriately maintained, code retrieval methods are guaranteed to generate curated code written by human developers, and hence a certain level of code quality can be guaranteed.
On the other hand, because they are fundamentally limited to only generating code that is included in the retrieval database, most of the time developers will further edit and adapt the snippet they searched to suit their specific context and need.
In contrast, code generation models can theoretically reduce this editing burden, but also do not necessarily guarantee that the generated code is semantically coherent or executable.
Because of this, in this work we examine a hybrid interface that is able to handle both modalities for obtaining code from natural language queries.

\subsection{Evaluation of Natural Language to Code Methods}
From the above sections, it is clear that there is a wide variety of methods that take in a natural language intent and output code, but how do we evaluate whether such methods are succeeding at their task?

In order to do so, the most common way is to create a ``reference'' program that indeed implements the desired functionality, and measure the similarity of the generated program to this reference program.
Because deciding whether two programs are equivalent is, in the general case, undecidable~\cite{rice1953classes}, alternative means are necessary.
For code generation in limited domains, this is often done by creating a small number of input-output examples and making sure that the generated program returns the same values as the reference program over these tests~\cite{zelle1996learning,berant2013semantic,zettlemoyer2007online,wang2015building,yao2014information,zhong2017seq2sql,zavershynskyi2018naps,kulal2019spoc,zhong2020semantic}.
However, when scaling to broader domains, creating a thorough and comprehensive suite of test cases over programs that have a wide variety of assumptions about the input and output data formats is not trivial.

As a result, much research work on code generation and retrieval take a different tack.
Specifically, many code generation methods \cite{yin2017syntactic,Iyer2018MappingLT,Agashe2019JuICeAL,xu2020incorporating} aim to directly compare generated code snippets against ground truth snippets, using token sequence comparison metrics borrowed from machine translation tasks, such as BLEU score~\cite{Papineni2002BleuAM}.
However, many code snippets are equivalent in functionality but differ quite largely in terms of token sequences, or differ only slightly in token sequence but greatly in functionality, and thus BLEU is an imperfect metric of correctness of a source code snippet~\cite{tran2019does}.

Code retrieval, on the other hand, is the task of retrieving relevant code given a natural language query, that is related to other information retrieval tasks. 
Since code retrieval is often used to search for vague concepts and ideas, human-annotated relevance annotations are needed for evaluation.
The common methods used in research work~\cite{gu2018deep,Yao2018StaQCAS,husain2019codesearchnet} compare the retrieved code snippet candidates given a natural language query, with a human annotated list of code snippet relevance, using common automatic information retrieval metrics like NDCG, MRR, etc.~\cite{manning2008introduction}
The drawback of this evaluation method is that the cost of retrieval relevance annotation is high, and often requires experts in the specific area.
Also, since the candidate lists are usually long, only a few unique natural language queries could be annotated.
For example, one of the most recent large scale code search challenge  CodeSearchNet~\cite{husain2019codesearchnet} contains only 99 unique natural language queries, along with their corresponding code snippet relevance expert  annotations, leading to smaller coverage of real world development scenarios in evaluation.

Regardless of the automatic metrics above, in the end our final goal is to help developers in their task of writing code.
However, despite the fact that we were able to identify over 30 papers\footnote{We get the estimate of how many papers use such metrics by checking papers and leaderboard submissions.} that devise code generation or retrieval methods and evaluate using these metrics, few to none ask the fundamental question of whether these methods will be useful within the developer workflow.
This is the gap that we fill in this paper, both by performing the first comprehensive study of modern techniques for code generation in the developer workflow, and by developing and releasing code for an experimental protocol that can be used in validation of future techniques for code generation or retrieval.


% Although we see little effect from the plugin on the efficiency, correctness, and complexity, we are interested about other effects \emph{among} the different queries in our hybrid approach.
% Thus, we ask the question: what kind of code is conducive to being written with the aid of code generation vs. code retrieval.

% Based on the background knowledge about both code generation and code retrieval described in Section~\ref{sec:background} \gn{missing section}, we expect that the users are more likely to use the code retrieval for the single query that contains complex intents that would usually requires multiple steps and sub-queries to fulfill, because this way the user would get more ``free code'' from the longer retrieved snippets.
% Besides, if users are familiar with using web search engines to search for programming questions, their queries may be more suited to a code retrieval approach (which requires less specified queries) than a generation approach (which requires more specified queries) \gn{updated this sentence, please check}.

% \gn{I would've expected this paragraph to be about the \emph{positive} parts of code generation, given the previous paragraph was about the positive parts of code retrieval. Please consider rewriting this.}
% Looking back at code generation, the code generation model's training data usually contains mostly simpler programming intents than full-blown functions, such as data analysis or visualization code.
% The model capacity may also be another limiting factor.
% We also think that the code generation model can only generate code containing the equivalent amount of information described in the natural language query, and thus when queries are short, fully-specified and clear, they work well, but when queries are multihop, under-specified, they are not as good as the retrieval results.


% After data filtering and cleaning process in Section~\ref{sec:datafilter}, we obtained 225 data points for task completion time analysis.
% Among them, 106 data points do not use the plugin, and the remaining 119 data points use the plugin.

% \begin{figure}[t]
%      \centering
%     \includegraphics[width=\textwidth]{figures/completion_time/completion_time_violin.pdf}
%     \caption{Split violin plots for all tasks as well as each task category. Each compares the two distributions representing the task completion time when using the plugin and not using the plugin. Time is in seconds.}
%     \label{fig:completion_time_category}
% \end{figure}

% Looking into more detail, from the rest of  Figure~\ref{fig:completion_time_category}, we can see detailed comparison for each task category.
% Note that some task categories like Web Scraping and Web Server \& Client have very few participants and thus the results for them are not conclusive.
% Besides these, we can see that some task categories like Basic Python, File, Data Analysis \& Machine Learning, the mean completion time using the plugin is somewhat lower than when not using the plugin, but due to the small sample size of these subdivided datasets, the values are not statistically significant ($p > 0.05$) and thus we can not conclude whether this is a real effect or result of randomness.

% \subsection{Results: Program Correctness}
% \label{sec:results_task_correctness}

% {\footnotesize \input{lmer_program_correctness} }

% \bv{To do: Add and discuss model table. Revise text}

% After the data filtering and cleaning process, we obtained 237 data points for task completion correctness analysis.
% Among them, 111 data points do not use the plugin, and the rest 126 data points use the plugin.


% \begin{figure}[t]
%      \centering
%     \includegraphics[width=\textwidth]{figures/score/score_violin.pdf}
%         \caption{Split violin plots for all tasks as well as each task category. Each compares the two distributions representing the task correctness score when using the plugin and not using the plugin. Score ranges from 0 to 10.}
%         \label{fig:score_category}
% \end{figure}

% Looking into more detail, from the rest of  Figure~\ref{fig:score_category}, we can see detailed comparison for each task category.
% Note that similar to the situation of completion time, some task categories like Web Scraping and Web Server \& Client have very few participants and thus the results for them are not conclusive.
% Besides these, we can see that in some task categories like File, OS \& Data Visualization tasks, the plugin is somewhat helpful in terms of correctness scores, but not statistically significant ($p > 0.05$) when we test them.

% However, comparing the correctness scores with completion time, we find that the p-value for scores is lower than completion time, suggesting that the plugin usage might have a bigger effect on potentially improving correctness than improving efficiency.
% We also find that among 7 categories, the plugin affects task completion time and correctness differently, as for some categories like the OS, the efficiency is indistinguishable, but more noticeable in correctness.


% \subsection{Results: Code Complexity}
% \label{sec:results_complexity}

% {\footnotesize \input{lmer_code_complexity} }

% \bv{To do: Add and discuss model table. Revise text}


% We obtain 237 data points for cyclomatic complexity analysis.
% Among them, 111 data points do not use the plugin, and the rest 126 data points use the plugin.

% For the group using the plugin, the complexity statistics are: Min.: 1.000, 1st Qu.: 2.000, Median: 3.500, Mean: 5.135, 3rd Qu.: 6.000, Max.: 50.000.
% For the group not using the plugin, the complexity statistics are: Min.: 1.000, 1st Qu.: 1.000, Median: 3.000, Mean: 4.279, 3rd Qu.: 6.000, Max.: 18.000.

% From Figure~\ref{fig:cc_category}, we can see that overall, the complexity score is not very different between the two distributions.
% There are also a lof of outliers.
% We then perform the Welch Two Sample t-test and find that the two distributions are not significantly different in means ($p = 0.181$).

% We then fit the linear mixed effects model where we treat user and task as random effects.
% For the fixed variable that we are interested in: using the plugin, the coefficient is 0.73 ($p = 0.206$), suggesting no significant relationship between using the plugin or not, with regard to the code complexity.

% \begin{figure}[t]
%      \centering
%     \includegraphics[width=\textwidth]{figures/cc/complexity_violin.pdf}
%         \caption{Split violin plots for all tasks as well as each task category. Each compares the two distributions representing the code complexity score when using the plugin and not using the plugin.}
%         \label{fig:cc_category}
% \end{figure}

% Looking into more detail, from the rest of  Figure~\ref{fig:cc_category}, we can see detailed comparison for each task category.
% Besides some task categories like Web Scraping and Web Server \& Client that have very few data points and thus whose results are not conclusive, we can see that complexity scores are not effected by the plugin, and if anything, the difference between the means is statistically insignificant ($p > 0.05$) when we test them.





% In our first research question, we ask about the effect on
% How does the incorporation of such an interface affect programmer efficiency, resulting program correctness, or code quality?

% \gn{Sections 4.1-4.3 seem a bit redundant, there are several places where the structure is quite similar between the sections and phrases seem to overlap.
% It seems like it might be better to combine all of them together in some way. For example, have 4.1 be description of the speed, correctness, and complexity metrics, 4.2 be a description of the analysis techniques, and 4.3 be a description of the results.
% This would also help compare and contrast between the different results.
% }
% \fx{@Bogdan, could you help look at Graham's comment here?}

% \subsection{Task Completion Time}
% \label{sec:method_completion_time}

% \subsubsection{Approach}
% First, we examine the effect of the plugin on the task completion time, i.e.~efficiency.
% Based on the user activity logging inside the VM, we can calculate the actual time used by the user to complete a given task.
% Specifically, we calculate the time interval based on the start time and final submission time of the assignment, and subtract any time occurred during the user using the pause/resume functionality during the user study process.
% To further increase the accuracy of the estimation of the completion time, we also deduct all the idle time when the user has no mouse or keyboard activity for more than 2 minutes, using our collected keystroke and mouse movement data inside the environment.
% After all these, we have a more accurate task completion time for each assignment.
% We also remove data points where unexpected errors (missing logs, inconsistent logs, etc.) happen during the logging process leading to incorrect task completion time calculations.

% After data filtering and cleaning process in Section~\ref{sec:datafilter}, we obtained 225 data points for task completion time analysis.
% Among them, 106 data points do not use the plugin, and the remaining 119 data points use the plugin.

% Obtaining the 2 distributions, we visualize the two distributions both as a whole and separately for each task category.
% We perform Welch's t-test~\cite{welch1947generalization} between the two distributions to see if the two groups' means are statistically significantly different.
% To further understand the underlying factors that may have effects on the task completion time, we fit a linear mixed-effects model~\cite{lindstrom1988newton} to the data.
% Linear mixed models are an extension of simple linear models to allow both fixed and random effects, and are particularly used when there is non-independence in the data.
% The key components in the mixed models are fixed and random effects.
% A fixed effect is a parameter that does not vary, while in contrast, random effects are parameters that are themselves random variables.
% Formally, The model will be:
% \begin{align}
%     y = \beta_1x_1 + ... + \beta_mx_m + u_1z_1 + ... + u_nz_n + \epsilon 
% \end{align}
% where $y$ is the outcome variable, and it depends on $m$ fixed effects $x_i$ and their corresponding fixed-effects regression coefficients $\beta_i$, as well as $n$ random effects $z_i$ and their corresponding random complement $u_i$ to the fixed $\beta_i$.

% Since we are interested in how the plugin use would effect the task completion time, 
% we first consider a basic model where plugin use is the fixed effect, with user and task as random effects, formulated as:
% \begin{align}
%     \texttt{completion\_time} = \beta_1\texttt{use\_plugin} + u_1\texttt{user} + u_2\texttt{task} + \epsilon 
% \end{align}
% where $\beta_i$ is the coefficient for the fixed effects and $u_i$ is the coefficient for the random effects.
% The intuition behind using user and task as random effects is to try to eliminate the confounding factors where different users may have different expertise in different tasks, as well as different tasks have varying difficulties.

% \subsubsection{Results}
% \gn{This is a lot of detail for the main text, maybe it can just be deleted, the figure is probably sufficient.}
% For the group using the plugin, the task completion time statistics (in seconds) are: Min.: 36, 1st Qu.: 1054, Median: 1698, Mean: 2510, 3rd Qu.: 3136, Max.: 9900.
% For the group not using the plugin, the task completion time statistics (in seconds) are: Min.: 211, 1st Qu.: 1057, Median: 2240, Mean: 2817, 3rd Qu.: 3714, Max.: 9986.

% From Figure~\ref{fig:completion_time_category}, we can see that overall, the average time taken to complete the task when using the plugin is similar to that without.
% We then perform the Welch Two Sample t-test and find that the two distributions are not significantly different in means ($p = 0.3058$).

% We then fit the linear mixed effects model where we treat user and task as random effects.
% For the fixed variable that we are interested in: using the plugin, the coefficient is -47.56 ($p = 0.811$), suggesting that no significant difference in task completion time between using the plugin or not.

% \begin{figure}[t]
%      \centering
%     \includegraphics[width=\textwidth]{figures/completion_time/completion_time_violin.pdf}
%     \caption{Split violin plots for all tasks as well as each task category. Each compares the two distributions representing the task completion time when using the plugin and not using the plugin. Time is in seconds.}
%     \label{fig:completion_time_category}
% \end{figure}

% Looking into more detail, from the rest of  Figure~\ref{fig:completion_time_category}, we can see detailed comparison for each task category.
% Note that some task categories like Web Scraping and Web Server \& Client have very few participants and thus the results for them are not conclusive.
% Besides these, we can see that some task categories like Basic Python, File, Data Analysis \& Machine Learning, the mean completion time using the plugin is somewhat lower than when not using the plugin, but due to the small sample size of these subdivided datasets, the values are not statistically significant ($p > 0.05$) and thus we can not conclude whether this is a real effect or result of randomness.

% One possible reasons why the plugin does not show effectiveness in improving completion time is that the user would still need time to figure out the queries for the plugin the either generate or retrieve. While the workflow integration may make it more efficient, many auto-inserted code snippets still need further editing, since the code generation model is far from perfect.
% Sometimes, the user still needs to use a web browser to figure out which candidate is the correct or most suitable one under the current intent and context.
% All of these still take time during the development even with the plugin, especially for the developers with less experience.
% Another possible reason is that the user may need many queries of trials and errors to test the plugin before they are more used to such a new interface.
% These could potentially be alleviated by improvements to plugin design or model accuracy, as discussed further in Section \ref{sec:discussionimplications}.

% \subsection{The Effect on Task Correctness}
% \subsubsection{Approach}
% Besides analyzing the effect with regard to the task completion time, we are also interested in how using the plugin would affect the correctness with which the user finished the task and the program functions as intended.
% To quantify the correctness of the user's task submissions, we follow the common practice in computer science education~\cite{Dawood2013RubricBA,Catet2017ApplicationOT,Grover2018WhatWC}, where we design a rubric for each task and the graders assign a score to each submission according to the rubric.
% In our case, we design rubrics to cover the basic aspects (e.g. runs without errors/exceptions; produces the same output as the example output provided in the task description), and implementation details regarding functional correctness (e.g. considering edge cases, implementing all required functionality in the task description).
% We make our best effort to cover the common difficulties and questions used to create the tasks in the first place, as described in Section~\ref{sec:design}.
% For each item in the rubric a score is assigned, and the full score for each task is 10 points.
% The full rubrics can be found at \url{https://github.com/neulab/tranx-study/blob/master/rubrics.md} for reproducibility.

% For example, for the task described in Section~\ref{sec:design}, we create the following rubric, with the number in the parenthesis representing the points worth for the item:
% \begin{mdframed}[backgroundcolor=blue!10] 
%     \begin{enumerate}
%         \item Runs without errors (2)
%         \item Correct image format (png) output (2)
%         \item Read in the raw data file in correct data structure (1)
%         \item Correct plot size (1)
%         \item Correctly handle missing data points (1)
%         \item Date (x axis) label in correct format (1)
%         \item Title set correctly (1)
%         \item Font size and color set according to specification (1)
%     \end{enumerate}
% \end{mdframed}

% \gn{While reading through this paragraph and the following two paragraphs this felt like too much information, maybe this could be relegated to an appendix.}
% To ensure better reproducibility and reduce subjectivity, we score the rubrics automatically as much as possible.
% There are two main types of automatic scoring we use: the first being black-box testing where we test if the program could run without errors and judging from the output to test for each rubric.
% For example, one of the task asks to ``print the date and time one week from now in the GMT timezone, in the format of mm-dd-yyyy hh:mm (24hr format)'', we first check if the program runs without errors, then we parse to output to automatically check if it is in the correct datetime format, and then we check if it is one week from now, regardless of the timezone (considering UTC-12 to UTC+12 both correct), and eventually check if the output is actually representing GMT timezone.

% The second type of automatic scoring is white-box testing, where we parse the source code and apply pre-defined heuristics to the source code parse tree to check whether a desired functionality if correctly implemented as described in the rubrics.
% For example, some rubrics may require you to use dictionary as a data structure as specified in the task description, then we can check if the dictionary type is created and updated throughout the source code parse tree.
% Although there might be false positives or true negatives in the heuristics, we try our best effort to design the heuristics to minimize those, and leave the cases that are hard to create heuristic rules for to manual scoring.
% Those that need manual scoring include tasks that are not deterministic, like machine learning tasks, or  the data visualization tasks that output image files that is hard to evaluate automatically.

% Based on a combination of automatic grading and manual grading, we go through all the valid submissions and score each of them from 0 to 10 based on the rubric without knowing the user's information to ensure fair grading.
% Similarly to the process used before, we also filtered out data from users that rarely use the plugin throughout the whole user study.

% After obtaining distribution of the correctness scores over the two groups (use plugin or not), we run similar analysis as described above, including visualization in box plots, and Welch's t-test~\cite{welch1947generalization} for significance tests.
% Also, to understand the underlying factors that may have an effect on task correctness, we propose a linear mixed-effects model and fit them on the data by maximum likelihood, and perform significance tests with t-tests using Satterthwaite's method.

% Since we are interested in how the plugin use would effect the task correctness time, 
% we first consider a basic model where the plugin use is the fixed effect, with user and task as random effects, formulated as:
% \begin{align}
%     \texttt{correctness} = \beta_1\texttt{use\_plugin} + u_1\texttt{user} + u_2\texttt{task} + \epsilon 
% \end{align}
% where $\beta_i$ is the coefficient for the fixed effects and $u_i$ is the coefficient for the random effects.

% \subsubsection{Results}
% After the data filtering and cleaning process, we obtained 237 data points for task completion correctness analysis.
% Among them, 111 data points do not use the plugin, and the rest 126 data points use the plugin.

% % \gn{As suggested above, the results being part of the main text here seems sub-optimal.}
% % For the group using the plugin, the task correctness score statistics are: Min.: 1.000, 1st Qu.: 6.000, Median: 7.000, Mean: 7.111, 3rd Qu.: 9.750, Max.: 10.000.
% % For the group not using the plugin, the task correctness score statistics are: Min.: 1.000, 1st Qu.: 4.000, Median: 6.000, Mean: 6.586, 3rd Qu.: 9.000, Max.: 10.000.

% From Figure~\ref{fig:score_category}, we can see that overall, the correctness of the tasks using the plugin is better than that without.
% We then perform the Welch Two Sample t-test and find that the two distributions are not significantly different in means ($p = 0.1315$).

% We then fit the linear mixed effects model where we treat user and task as random effects.
% For the fixed variable that we are interested in: using the plugin, the coefficient is 0.44 ($p = 0.136$), suggesting no significant relationship between using the plugin or not, with regard to the correctness scores.

% \begin{figure}[t]
%      \centering
%     \includegraphics[width=\textwidth]{figures/score/score_violin.pdf}
%         \caption{Split violin plots for all tasks as well as each task category. Each compares the two distributions representing the task correctness score when using the plugin and not using the plugin. Score ranges from 0 to 10.}
%         \label{fig:score_category}
% \end{figure}

% Looking into more detail, from the rest of  Figure~\ref{fig:score_category}, we can see detailed comparison for each task category.
% Note that similar to the situation of completion time, some task categories like Web Scraping and Web Server \& Client have very few participants and thus the results for them are not conclusive.
% Besides these, we can see that in some task categories like File, OS \& Data Visualization tasks, the plugin is somewhat helpful in terms of correctness scores, but not statistically significant ($p > 0.05$) when we test them.

% However, comparing the correctness scores with completion time, we find that the p-value for scores is lower than completion time, suggesting that the plugin usage might have a bigger effect on potentially improving correctness than improving efficiency.
% We also find that among 7 categories, the plugin affects task completion time and correctness differently, as for some categories like the OS, the efficiency is indistinguishable, but more noticeable in correctness.

% One possible reason is that both code generation and retrieval will guarantee syntactic correctness of the inserted code.
% Furthermore, the retrieved code snippets are usually highly up-voted answers on Stack Overflow, and thus the snippets on their own have high credibility, and the only thing that the user should do is to correctly adopt the retrieved code to suit the need in context.


% \subsection{The Effect on Code Complexity}
% \subsubsection{Approach}
% In previous sub-sections, we discuss possible effects of using the plugin may have on programming \emph{efficiency} and \emph{correctness}.
% In real-world development scenarios, the code's maintainability is also an important factor to judge the quality of the code.
% We are interested in whether using the plugin would affect the maintainability, or complexity of the code.

% To automatically evaluate the complexity of the code (in the sense of source code complexity as opposed to algorithmic complexity), we calculate McCabe's cyclomatic complexity, a quantitative measure of the number of linearly independent paths through a program's source code.~\cite{McCabe1976ACM}
% This software metric can also imply ``structuredness'' in programs~\cite{Watson1996StructuredTA}.

% If we consider a structured program in the form of a control flow graph, a directed graph containing the basic blocks of the program, with an edge between two basic blocks if control may pass from the first to the second. The McCabe's cyclomatic complexity $M$ is then defined as:

% \begin{align}
%     M = E - N + 2P
% \end{align}
% where $E$ is the number of edges of the graph, $N$ is the number of nodes of the graph, and $P$ is the number of connected components.
% In real programs, the complexity depends a lot on the ``if''-statements, as well as conditional loops, and whether these are nested.
% We use an open-source library Radon~\footnote{\url{https://github.com/rubik/radon}} to calculate the total Cyclomatic Complexity for each submitted program's source code file.

% After obtaining the two groups (use plugin or not) distribution of the complexity scores, we again run similar analysis as described above, including visualization in box plots, Welch's t-test~\cite{welch1947generalization} for significance tests.
% Also, to understand the underlying factors that may have effects on the task completion correctness, we propose a linear mixed-effects model and fit them on the data by maximum likelihood, and perform significance tests with t-tests using Satterthwaite's method.

% Similarly to above, we are interested in how the plugin use would effect the task correctness time, 
% we consider a basic model where the plugin use is the fixed effect, with user and task as random effects, formulated as:
% \begin{align}
%     \texttt{complexity} = \beta_1\texttt{use\_plugin} + u_1\texttt{user} + u_2\texttt{task} + \epsilon 
% \end{align}
% where $\beta_i$ is the coefficient for the fixed effects and $u_i$ is the coefficient for the random effects.

% \subsubsection{Results}
% We obtain 237 data points for cyclomatic complexity analysis.
% Among them, 111 data points do not use the plugin, and the rest 126 data points use the plugin.

% % For the group using the plugin, the complexity statistics are: Min.: 1.000, 1st Qu.: 2.000, Median: 3.500, Mean: 5.135, 3rd Qu.: 6.000, Max.: 50.000.
% % For the group not using the plugin, the complexity statistics are: Min.: 1.000, 1st Qu.: 1.000, Median: 3.000, Mean: 4.279, 3rd Qu.: 6.000, Max.: 18.000.

% From Figure~\ref{fig:cc_category}, we can see that overall, the complexity score is not very different between the two distributions.
% There are also a lof of outliers.
% We then perform the Welch Two Sample t-test and find that the two distributions are not significantly different in means ($p = 0.181$).

% We then fit the linear mixed effects model where we treat user and task as random effects.
% For the fixed variable that we are interested in: using the plugin, the coefficient is 0.73 ($p = 0.206$), suggesting no significant relationship between using the plugin or not, with regard to the code complexity.

% \begin{figure}[t]
%      \centering
%     \includegraphics[width=\textwidth]{figures/cc/complexity_violin.pdf}
%         \caption{Split violin plots for all tasks as well as each task category. Each compares the two distributions representing the code complexity score when using the plugin and not using the plugin.}
%         \label{fig:cc_category}
% \end{figure}

% Looking into more detail, from the rest of  Figure~\ref{fig:cc_category}, we can see detailed comparison for each task category.
% Besides some task categories like Web Scraping and Web Server \& Client that have very few data points and thus whose results are not conclusive, we can see that complexity scores are not effected by the plugin, and if anything, the difference between the means is statistically insignificant ($p > 0.05$) when we test them.

% We find that the complexity scores produce a lot of outliers in the distribution, with most of the programs written having a low complexity, while some cases have a very large complexity score due to the fact that some users' submissions are always re-implementing the wheels and have a lot of duplicate code for similar basic functionalities.
% For our designed tasks, the ideal program should indeed have low complexity since these are designed to be completed in a short amount of time with a small amount of features.
% Because of this, the complexity score comparison between using the plugin and not using the plugin cannot accurately reflect scenarios with large projects, and currently the outliers are a major contributing factor to the skewed distributions, since most correct code in our case are of low complexity.
% Most tasks also do not require a extremely complex structures of code and programs are usually linear.

% \RQ{types-of-code}{What kind of code is conducive to being written 
%     with the aid of the code generation vs.\ the code retrieval NL2Code assistant?}

% \input{queries}
% {\footnotesize
% \LTXtable{\linewidth}{queries}
% }



% After all assigned tasks are completed for the user, we asked them to complete a form about the overall experience with the user study and their evaluation of the plugin, additionally soliciting comments and suggestions.
% The details of the survey questions can be found in .

% The surveys are designed to get a grasp of how the users think the experience of code generation approaches integrated in their developing workflow and investigate research questions about the gap between idea scenarios with the current status.

% \mysec{Data Processing \& Filtering}
% % \label{sec:datafilter}
% To investigate the effects that using the proposed plugin may have on various dependent variables representing developer performance, we group all the valid submissions into two groups, ``plugin'' and ``no\_plugin'', representing whether or not the user used the plugin during the assignment.
% Although we assign each user whether or not to use the plugin for each task they are assigned by enabling/disabling the plugin automatically during the user study, a few users rarely use the plugin under either circumstances throughout the whole user study process.
% To solve this, we filter out all the data from the users that in total (during the whole user study) queried the plugin for less than 4 times. 



% During the user study process, we collected a variety of data from the user study, including:
% \begin{enumerate}
%     \item The user's interaction with the plugin in PyCharm IDE, including queries, candidate selections and edits.
%     \item The user's fine-grained IDE edit activities.
%     \item The user's web search/browsing activities inside the VM's Firefox web browser.
%     \item The user's keystrokes inside the VM.
%     \item The user's completed task program submissions.
% \end{enumerate}

% Specifically, to collect user's edit activities, whenever the user does not make modifications to the code for 1.5 seconds, the plugin uploads the current snapshot of the code to the server.
% The intuition behind this heuristic is that after the user makes some type of meaningful edit like adding or modifying an argument, variable, or function, they usually pause for a short time before the next edit.
% This edit activity granularity is more meaningful than keystroke/character level, yet finer than intent level or commit level edits.
% This data could also be helpful for future researchers to model developers' edit activities for automatic code generation or repair.

% More details of the design of the user study environment that allows participants to easily take part in the study and collect all the data possible are described in Appendix~\ref{app:environment_design}. 
% Besides releasing all the collected data to the public for future empirical research purposes after data anonymization, we use them to perform several analyses trying to answer our proposed research questions in the following sections.

% \subsection{Task Design}
% \label{sec:design}

% \gn{I changed some of the wording of this part that describes stuff that we did to past tense, but the other places probably should as well.}

% To emulate real world Python development activities, but to also fit the scope of the user study, we created a total of 14 reasonably sized tasks for assignment to the participants to complete.
% To design tasks that could cover most of the Python development scenarios, we first determined several categories of tasks that many use Python to implement. 
% Specifically, we browsed through several popular coding education websites, including Udacity\footnote{\url{https://www.udacity.com/courses/all}}, Codecademy\footnote{\url{https://www.codecademy.com/catalog}}, Coursera\footnote{\url{https://www.coursera.org/}}, etc. and searched for keyword ``Python'' and manually went through the results lists of courses.
% By aggregating the courses, we designed 7 categories that are most commonly taught regarding Python programming, indicating common use cases of Python programming language, with some of them using popular libraries in Python:
% \begin{enumerate}
%     \item Basic Python
%     \item File
%     \item OS
%     \item Web Scraping (e.g. \texttt{beautifulsoup})
%     \item Web Server \& Client (e.g. \texttt{requests, flask, django})
%     \item Data Analysis \& Machine Learning (e.g. \texttt{pandas, sklearn})
%     \item Data Visualization (e.g. \texttt{matplotlib})
% \end{enumerate}
% These were also selected based on two criteria: they should (1) be well-represented in the most frequently upvoted questions with the "python" tag on Stack Overflow, and (2) be diverse and cover a wide range of skills a developer may need.

% \bv{Defensive paragraph.}

% For each of the categories (or genres), we design 2 tasks covering most frequently asked questions and use cases.
% We look at the most frequently upvoted questions corresponding to that genre, usually by searching for the "python" keyword and another keyword (e.g. "python matplotlib", "python pandas"), select only questions that were asking how to do something (i.e. excluding questions that ask about features of the language, or about how to install packages), and try to devise tasks that would cover 3-5 of the most frequently upvoted questions.
% An example of such a task for the category ``Data Visualization (e.g. \texttt{matplotlib})'', represented by this search \url{https://stackoverflow.com/search?tab=votes&q=python%20matplotlib}, would be
% described as:

% \begin{mdframed}[backgroundcolor=blue!10] 
% By running \texttt{python3 main.py}, draw a scatter plot of the data in \texttt{shampoo.csv} and save it to \texttt{shampoo.png}. 
% The plot size should be with a size of 10 inches wide and 6 inches high. 
% The \texttt{Date} column is the x axis (some dates are missing from the data and in the plot the x axis should be completed with all missing dates without sales data).
% The date string shown on the plot should be in format \texttt{(YYYY-MM-DD)}. 
% The \texttt{Sales} column is the y axis. 
% The graph should have the title ``Shampoo Sales Trend''. 
% The font size of the title, axis labels, and x \& y tick values should be 20pt, 16pt, and 12pt respectively. 
% The scatter color should be in \texttt{purple}.
% \end{mdframed}

% This covers some of the top questions regarding data visualization with \texttt{matplotlib} found on Stack Overflow through the approach described above:
% \begin{enumerate}
%     \item How do you change the size of figures drawn with matplotlib?\footnote{\url{https://stackoverflow.com/questions/332289/how-do-you-change-the-size-of-figures-drawn-with-matplotlib}}
%     \item How to put the legend out of the plot?\footnote{\url{https://stackoverflow.com/questions/4700614/how-to-put-the-legend-out-of-the-plot}}
%     \item Save plot to image file instead of displaying it using Matplotlib?\footnote{\url{https://stackoverflow.com/questions/9622163/save-plot-to-image-file-instead-of-displaying-it-using-matplotlib}}
%     \item How do I set the figure title and axes labels font size in Matplotlib?\footnote{\url{https://stackoverflow.com/questions/12444716/how-do-i-set-the-figure-title-and-axes-labels-font-size-in-matplotlib}}
% \end{enumerate}
% For each task designed, we also provide the user with required input data or directory structure for their program to work on, as well as example outputs (console print-outs, output files \& directories, etc.) so that they could verify their programs during the user study.
% The tasks have varying difficulties, and on average each task would take about 15-40 minutes to complete.
% The full task descriptions and input/output examples for all 14 tasks can be found at \url{https://github.com/neulab/tranx-study} for reproducibility.


% \subsection{Participants \& Task Assignments}
% To recruit participants with varying development backgrounds, we put recruitment advertisements both inside the university community, as well as on a freelancer platform, Upwork.\footnote{\url{https://www.upwork.com/}}
% We aimed for the university community to attract students in computer science or related areas as well as researchers, and aimed for the freelancer platform to attract software engineers and data scientists.
% For each of the prospective participants, we asked them about two parts of the information in a pre-study survey, apart from personal information for contact purposes.
% The first is regarding programming experience, used to determine if the participants have enough expertise in Python as well as the categories of tasks that we designed.
% The questions are:
% \begin{enumerate}
%     \item Which of the following best describes your current career status: Student (computer science), Student (other field), Software Engineer, Data Scientist, Researcher, Other.
%     \item How do you estimate your programming experience? (1: very inexperienced to 5: very experienced)
%     \item How experienced are you with Python? (1: very inexperienced to 5: very experienced)
%     \item How experienced are you with each of the following tasks in Python? (1: very inexperienced to 5: very experienced) Basic Python, File, OS, Web Scraping, Web Server \& Client, Data Analysis \& Machine Learning, Data Visualization.
% \end{enumerate}
% The second part of the information is about their development preferences, used to ask for their preferences with IDE and assistive tools.
% The questions are:
% \begin{enumerate}
%     \item What editor/IDE do you use for Python projects? Vim, Emacs, VSCode, PyCharm, Jupyter Notebook, Sublime Text, other.
%     \item Do you use any assistive tools or plugins to improve your coding efficiency? Some examples are code linting, type checking, snippet search tools, etc. If yes, what are they?
% \end{enumerate}

% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[width=0.5\textwidth]{figures/demographic/occupation.pdf}
% %     \caption{Occupation demographics of the participants completed the user study. \gn{Bigger fonts here and everywhere. (also maybe replace it by a table or just in text)}}
% %     \label{fig:demographic_occupation}
% % \end{figure}



% We deemed participants with programming experience and Python experience greater or equal than a score of 3 in the survey eligible for the study, which resulted in a total of 64 qualified participants.
% However, only 44 of them completed the user study.
% The backgrounds were relatively diverse; of the 44 participants, 19 (43.18\%) were software engineers and 14 (31.82\%) were computer science students, with the rest being data scientists (3, 6.82\%), researchers (2, 4.55\%), and other occupations (6, 13.64\%).

% From the participants' self-reported experience in Python programming as well as 7 specific fields of our tasks, we selected only participants with adequate Python experience for the user study.%
% \footnote{
% For two specific fields, Web Scraping and Web Server \& Client had few participants with significant experience, with majority of participants assessing themselves with score of 3 and less.
% Because of this, we can only assign tasks of the two categories to very few participants, resulting in few data points that could lead to inconclusive results in this two areas.
% Other than that, most participants have good experience in other fields of specialty.
% }
% The details of the distribution of participants' experience is shown in Appendix~\ref{app:particpants_experience}.

% For each eligible participant, we assigned tasks based on the categories where they have the most expertise based on the survey responses.
% We assign each participants 4 categories (8 tasks) out of all 7 categories (14 tasks) based on the following criteria:
% \begin{enumerate}
%     \item Almost everyone eligible for the user study was experienced enough in the first 2 task categories (basic python, and file) so we assign everyone with 4 tasks under these 2 categories.
%     \item For the rest of the 5 categories, we rank them based on the participant's response the their experience regarding the task genre.
%     We then assign top 2 most experienced categories to the participant. 
% \end{enumerate}
% With this, each eligible participant had 4 categories assigned in total.
% To measure the plugin's effect while controlling for programming experience and task expertise, the we either enable or disable the plugin \emph{once} (out of 2 tasks) within each high-level task category (e.g. if it is on for task1-1, it should be off for task1-2).
% We inform the participant whether the plugin is on or off for any particular task, and ask them to attempt to use the plugin when it is available.%
% \footnote{Despite these instructions, some participants did not use the plugin when it was available, and thus we filtered out any participants that did not use the plugin at least 4 times.}

% \subsection{Post-study Surveys}
% \label{sec:postsurvey}
% To collect subjective impressions from the participants, we administered surveys after the whole user study was concluded.
% After all assigned tasks are completed for the user, we asked them to complete a form about the overall experience with the user study and their evaluation of the plugin, additionally soliciting comments and suggestions.
% The details of the survey questions can be found in Appendix~\ref{app:post_survey_details}.

% % The surveys are designed to get a grasp of how the users think the experience of code generation approaches integrated in their developing workflow and investigate research questions about the gap between idea scenarios with the current status.

% \subsection{Data Processing \& Filtering}
% \label{sec:datafilter}
% To investigate the effects that using the proposed plugin may have on various dependent variables representing developer performance, we group all the valid submissions into two groups, ``plugin'' and ``no\_plugin'', representing whether or not the user used the plugin during the assignment.
% Although we assign each user whether or not to use the plugin for each task they are assigned by enabling/disabling the plugin automatically during the user study, a few users rarely use the plugin under either circumstances throughout the whole user study process.
% To solve this, we filter out all the data from the users that in total (during the whole user study) queried the plugin for less than 4 times. 

% \begin{itemize}
%     \item \RQ{task-performance}{How does using a NL2Code developer assistant 
%     affect task completion time, program correctness, and code complexity?}
%     \item \RQ{types-of-code}{What kind of code is conducive to being written 
%     with the aid of the code generation vs.\ the code retrieval NL2Code assistant?}
%     \item \RQ{opinions}{How do users perceive the usefulness of the two in-IDE 
%     NL2Code developer assistants?}
% \end{itemize}


% This section describes our study design and experimental environment.
% In order to perform an objective and replicable study we followed the guidelines
% on empirical software engineering in~\cite{wohlin2012experimentation,shull2007guide}.
% In order to allow independent verification and replication of the performed study, or allow application to the evaluation of future code generation methods, we make publicly available our plugin prototype, user study environment, code for data extraction and analysis, as well as the obtained anonymized raw data.


% The study includes 14 Python programming tasks in 7 categories with varying difficulty and focus, completed by 44 developers with diverse background in a controlled setting (i.e., some use the plugin while some do not during some tasks) with comprehensive data collection that took a total of over 170 person hours.
% An overview of the study process is shown in Figure~\ref{fig:overview}, and in the following subsections we introduce key design components of this.




% \section{Study Design}
% This section describes our study design and experimental environment.
% In order to perform an objective and replicable study we followed the guidelines
% on empirical software engineering in~\cite{wohlin2012experimentation,shull2007guide}.
% In order to allow independent verification and replication of the performed study, or allow application to the evaluation of future code generation methods, we make publicly available our plugin prototype, user study environment, code for data extraction and analysis, as well as the obtained anonymized raw data.


% % \gn{I commented out the first sentence here because it's basically already explained in the intro.}
% % \subsection{Goal \& Overview}
% % \label{sec:rq}
% % The goal of our study is to understand how using an intelligent natural language programming interface would affect developers' coding experience, for the purpose of gaining insight on the gap between the purported capabilities of code generation/retrieval models and real world needs.
% The study includes 14 Python programming tasks in 7 categories with varying difficulty and focus, completed by 44 developers with diverse background in a controlled setting (i.e., some use the plugin while some do not during some tasks) with comprehensive data collection that took a total of over 170 person hours.
% An overview of the study process is shown in Figure~\ref{fig:overview}, and in the following subsections we introduce key design components of this.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/overview.pdf}
%     \caption{An overview of the user study process. \gn{Add mapping from the collected data to individual RQs}}
%     \label{fig:overview}
% \end{figure}


% abstract syntax trees of the target code snippets; when instantiated for Python,
% the model can generate short code snippets given English descriptions of
% intent, \eg the code snippet ``\texttt{x.sort(reverse=True)}'' given the
% natural language input ``sort list \texttt{x} in reverse order''.

% Similarly, \citet{Iyer2018MappingLT} proposed a system to generate class 
% member functions given natural language descriptions of intent and the 
% programmatic context provided by the rest of the class.
% Finally, \citet{Agashe2019JuICeAL} proposed a system to generate the API 
% call sequence in a Jupyter Notebook code cell given the natural language 
% and code history up to that particular cell.
% We are still a ways away from not having to write any code while programming, 
% but all these systems reportedly have reasonable accuracy on benchmark datasets, 
% which makes our research study of their practical usefulness timely.


% Even though these systems focus on slightly different tasks, they are 
% conceptually similar to the aforementioned approach by \citet{yin2018tranx}
% in their design (comparable neural network architectures) and they achieve 
% comparable levels of accuracy. \bv{Is this true?}
% We choose to use the \citet{yin2018tranx} approach in our human study as one element 
% of our NL2Code plugin because of our familiarity with the implementation
% and the natural complementarity with code retrieval, discussed below.
% % models as one element of our interface, along with code retrieval, below.

% For example, given the natural language input ``sort list \texttt{x} in reverse order'', 
% one can expect based on current technology~\cite{yin2017syntactic,yin2018tranx} 
% the Python output ``\texttt{x.sort(reverse=True)}'' to be automatically generated.
% These systems are quite sophisticated, involving a syntactic tree-based neural 
% network model that encodes natural language utterances and generates abstract 
% syntax trees of the target code snippets; they have been trained on both official 
% API documentation and Stack Overflow questions and answers~\cite{xu2020incorporating}; 
% and they can generate reasonable code fragments given short text inputs, as 
% shown in Table~\ref{tab:case}.
% Note how such models can generate syntactically correct code snippets by
% construction; demonstrate ability to identify and incorporate a wide variety 
% of API calls; and also have the ability to copy important information like 
% string literals and variable names from the input natural language intent.


% The rest of this paper is organized as follows:
% We give some background on NL2Code approaches and discuss relevant related
% work in Section~\ref{sec:background}, ...


% The \textbf{target audience} of this paper is composed of Python developers, researchers from software engineering community, as well as researchers from machine learning community.
% We support Python developers by providing them with a prototype plugin of intelligent natural language programming interface for improving daily programming experience in PyCharm IDE.
% We support researchers from software engineering community by (i) providing a characterization of the developers' interaction with such interface, (ii) providing comprehensive data collected and open issues derived from the study.
% We support researchers from machine learning community by (i) providing developer edits with the generated or retrieved code for model improvements,
% (ii) feedback from developers' usage of such interface and elicit the real-world needs of the model, (iii) providing a user research tool, harness and environment that could be used to test future models in real world.

% The remainder of this paper is structured as follows. Section 2 ...

% In this paper, we aim to assess whether an intelligent interfaces using current state-of-the-art techniques for code generation and search are beneficial within the developer workflow, and also elucidate the advantages and disadvantages of code retrieval- and generation-based approaches.
% We propose the following research questions:
% \begin{itemize}
    % \item \textbf{RQ1}: How does the incorporation of such an interface affect programmer efficiency, resulting program correctness, or code quality?
    % \item \textbf{RQ2}: What kind of code is conducive to being written with the aid of code generation vs. code retrieval?
    % \item \textbf{RQ3}: How does the incorporation of a code generation and retrieval interface into the developer pipeline affect subjective user experience?
% \end{itemize}
% We answer the questions by empirically analyzing the developers' performance and activities when using or not using these assistive tools.

% \gn{This seems like a bit too much detail, perhaps compress to about half the size?}
% Specifically, we develop a plugin for the Python language in PyCharm IDE that combines results from both natural language to code generation and code retrieval.
% This is to cover both types of interactions of developers using natural language intents and commands to program mentioned above, and to put the state-of-the-art code generation model to a real world  test.
% It also reduces the amount of operations required for the developer to search for code snippets on the web, by integrating such procedure inside the plugin and the IDE's workflow.
% For assessment, we design 7 categories, a total of 14 common Python development tasks, ranging from basic Python to data science topics, with varying difficulties.
% We recruit 44 participants from various backgrounds to complete tasks in our controllable environments to collect multiple aspects of participants' interaction and activity events (e.g. web browsing, keystrokes, fine-grained code edits) for analysis.

% We also evaluate the efficiency of implementation and correctness of their task submissions, and analyze the effect of plugin usage on these variables.
% In addition to objective metrics, we also let the participants fill out questionnaires about their experience with the tasks and the plugin.
% To further investigate the differences between the two methods using natural language queries: code generation and code retrieval, we also analyze under what scenarios would the developer prefer code generation over code retrieval, or vice versa, and how many edits are needed to modify the retrieved or generated code snippets.

% As a result, we find that while developers in general enjoyed using the plugin within their development workflow, there were no quantitative gains in measurable outcomes such as developer efficiency, program correctness, or code quality.
% This indicates that despite impressive improvements in the intrinsic performance of code generation models, there may still be a need to further improve accuracy of code generation, and we may need to consider other extrinsic factors (such as providing documentation for the generated code) before the models make a notable impact on the developer workflow.

% plugin is far from perfect for real-world usage, we discuss the open issues lying in the current state of the natural language programming interface, and the ways that the data collected after the large-scale deployment of the plugin could improve code generation or code completion models in the future.

% Finally, we release all the collected data during the study, including detailed interaction events with the plugin, like queries and edits, web browsing activities, keystrokes, and fine-grained edits inside the IDE throughout the user study process. As~\cite{proksch2018enriched} suggests, such developer event stream data may benefit future empirical studies on developer activities. 




% Developers are human beings. Despite the fact that developers can ``speak'' programming languages to execute certain tasks, they can think, conceptualize, and communicate their intentions, command, and logic more easily using \emph{natural language}.
% One of the major difficulties of programming is turning \emph{concepts}, described in natural language, into \emph{code}, described in programming languages. 
% In fact, developers ask questions in natural language about how to perform these transformations all the time.
% For example, a quick search on Stack Overflow about Python\footnote{\url{https://stackoverflow.com/questions/tagged/python}} reveals developers asking questions such as ``How do I check whether a file exists without exceptions?'', or ``How do I merge two dictionaries in a single expression in Python (taking union of dictionaries)?''.
% % These questions are asked in natural language, describing the concept or logic that the developers wish to implement in the programming language of their choice.
% This difficulty is especially evident when dealing with unfamiliar APIs, and as a result developers also ask large number of questions about specific methods or function usages.
% % In fact, when presenting a programming library or new APIs, well-written and thorough documentations are much needed for the developers to understand the functionalities they are unfamiliar with.

% With this intuition, IDEs could make the life of developers easier if they could directly use \emph{natural language} commands to express their intent (sometimes called ``natural programming'')~\cite{myers2016programmers}.
% Many developers extensively search with natural language queries on the Internet for code snippets that fulfill such intents~\cite{Sim2013ACE,Ge2014HowDU,sadowski2015developers,Rahman2018EvaluatingHD,Tamla2019WhatDS}, and we call systems that provide this variety of natural language assistance \emph{code retrieval}.
% On the other hand, there has also been a recent focus on machine learning models that can generate new code snippets given natural language intents~\cite{Oda2015LearningTG,DBLP:conf/acl/RabinovichSK17,DBLP:conf/acl/LingBGHKWS16,Zhong2017Seq2SQLGS,Iyer2018MappingLT,xu2020incorporating,yin2018tranx,yin2017syntactic,Agashe2019JuICeAL}, which we refer to as \emph{code generation}.

% While research on both methods for creating appropriate code from natural language intents have received significant research interest in machine learning circles, there is a surprising paucity of work evaluating whether these methods are actually effective \emph{within the software development workflow}.
% Because of this, it is not necessarily clear that high automatic accuracy evaluation scores on benchmark datasets will directly translate to real-world usage scenarios when interacting with developers completing various development tasks.
% For example, an existing empirical study in code migration shows that automatic scores used in natural language translation (e.g. BLEU~\cite{Papineni2002BleuAM}) have only weak correlation with the semantic correctness of translated code~\cite{tran2019does}.



% Out of the sampled \numoraclequeries queries, 38\% end up being selected by the user with the code generation candidate.
% 40\% of the queries are deemed ``good on its own'' following the manual query analysis procedure, and 68\% of the queries are deemed ``good with context''.
% Note that here ``good with context'' also includes all queries that are ``good on its own''.
% This is expected as code generation is not perfect and cannot handle all the well-defined queries, and it is also expected that some queries issued by the user are implicitly ignoring key information in the current code context at the time, as the user are assuming them.
% Without the context information, the query is usually under-specified and thus the code generation model would not perform as well.

% Furthermore, we look at the correlation between the individual queries that are ``good on its own'' or ``good with context'', and those result in successful code generations.
% The Phi coefficient between whether the queries are ``good on its own'' and  whether the queries end up producing successful code generation results is 0.370 (p<0.05), suggesting moderate positive relationship.
% The Phi coefficient between whether the queries are ``good with context'' and whether the queries end up producing successful code generation results is 0.449 (p<0.05), suggesting strong positive relationship.
% From the positive correlation, we conclude that better query formulation is very crucial to the success of the code generation performance.

% \subsubsection{Approach}
% We examine representative features that make particular types of natural language queries result in more favorable code snippets (selected by the user) from code generation than code retrieval and vice versa.
% Through our user study harness, we collect all queries issued by the users as well as the final selection of the listed candidates (both generated and retrieved code snippets).
% Note that we ignore queries that the user did not select any candidates, as these candidates are deemed low quality, regardless of code generation or retrieval results.
% We now have a dataset containing natural language queries and their corresponding candidate selection type: either from generation or from retrieval.
% We treat the category of the candidate the user ended up using as the more favorable means, among generation and retrieval, to respond to such queries.

% To analyze the factors contributing to the final choice, we propose a simple analysis method where we train an interpretable classification model to predict, given features of the input query, whether generation or prediction result is selected.
% We first represent each natural language query using a bag-of-words vector, which is a vector representation of text where each element of the vector corresponds to the number of times a particular word occurred in the query.
% \gn{The following seemed overly verbose}
% It involves a vocabulary of known words over the corpus and a measure of the presence of known words.
% In other words, in this approach, we look at the histogram of the words within the text, i.e. considering each word count as a feature, and represent the whole query as vector with word count as elements, with the dimension of the size of the vocabulary.

% We use logistic regression model to predict one of the two labels given the query representation vector: whether the user picked generated code, or retrieved code.
% The logistic regression model is formulated as:
% \begin{align}
% \label{logmod} 
% Pr(\text{query uses generated})&=\frac{\exp(\beta_{0}+\beta_{1}X_{1}+\ldots+\beta_{k}X_{k})}{1+\exp(\beta_{0}+\beta_{1}X_{1}+\ldots+\beta_{k}X_{k})}\notag \\ & =\frac{\exp(\textbf{X}\beta)}{1+\exp(\textbf{X}\beta)} 
% \end{align}
% Where $\textbf{X}$ here represents a $k$-dimensional bag-of-word vector representation of a given query, and $\beta$ are the parameters to be learned during the model training.
% We use 0.5 as a cutoff probability for our binary labels.

% We randomly split all the collected query and candidate selection pairs into training and test set, with 70\% used for training and 30\% used for testing.
% On the training set, we use cross-validation techniques to train the classification model until it converges.
% The intuition is that if the model trained can predict the source of the candidates that the user ends up selecting, then the word feature weights ($\beta$) used in the logistic regression model could shed some light on what features are the most representative of queries that were effectively answered using generation or retrieval.
% By analyzing the word weights, we try to come up with some common type of queries that are suitable for code generation and code retrieval, respectively.

% \subsubsection{Results}

% We have collected a total of 447 queries that successfully produced either generated code or retrieved code that was selected by the user.
% We tokenize the natural language queries and filter out English stop words to calculate the bag-of-words representation for each query.
% After training the logistic regression model, we tested the model on the held-out data and found it achieves 64.4\% accuracy, where a trivial model that always chose ``code generation'' would achieve 55.6\% accuracy.
% This indicates that the model was able to learn some patterns of differences between those queries that are more suitable for code generation than code retrieval and vice versa.

% In Table~\ref{tab:query-class-features}, we show the top features that contributed to predicting one of the two categories, and their corresponding weights.
% We find that for code generation, the highest ranked features (tokens in the query sentence) contains mostly basic functionalities in Python, e.g. ``open, read, output'' (opening and reading a file), ``sort, list, number, dictionary, keys'' (related to basic data structures and operations in Python), ``random'' (related to the tasks that deals with randomness), ``trim'' (string operations), etc.
% These functionalities are basic but crucial in a wide variety of applications, and the fact that users prefer to use code generation model outputs as their selected candidates indicates that code generation provides effective options for these sorts of simpler functionalities.
% For example, some stereotypical queries containing these keywords that end up using the generated candidates are ``open a csv file \`{}data.csv\`{} and read the data'', ``get date and time in gmt'', ``list all text files in the data directory'', etc.
% Those that end up using retrieved candidates are ``generate random lower case letters'', ``copy all files and directories from one folder to another'', ``how to choose plot title in matplotlib'', ``sklearn cross validation x, y for 5 folds'', etc.

% On the other hand, we see that many queries that are more likely to be solved through code retrieval contains terms regarding more complex functionality to implement, some usually requiring a series of steps to fulfill.
% For example, ``datetime'' (regarding date and time operations), ``cross validation, sklearn, column'' (regarding machine learning and data analysis), ``matplotlib'' (data visualization), etc. are all among top features for queries suitable for code retrieval.
% This is an intuitive result, as the code retrieval model could find relevant code snippets, often quite long and complete, given only a few keywords describing the intent.

% Another interesting discovery is that the term ``python'' is also one of the highest weighted features for those end up using code retrieval. 
% Our reasoning is that the users have the habit of using web search engines to search for programming questions and help, so that they tend to always include ``python'' as a specifying keyword in those queries, even though this is not required in this particular code retrieval scenario.
% The results seen from the analysis are in line with our hypothesis in this section on the expected relative benefits of code retrieval and code generation.

% In summary, we find that both code generation and code retrieval could help different aspects of queries and intents in real use scenarios, and thus future research and development of both types of models would be valuable.

% \subsection{Manual Analysis of Query Quality}
% \subsubsection{Approach}
% We manually analyze what effects the formation of natural language queries may have on the eventual generation or retrieval candidate selection.
% This is also trying to answer how code generation and code retrieval methods would react to various quality of input natural language queries.

% The intuition behind this is that the developers are very used to how to search with search engines like Google and thus they do not put enough information into the query, or just use several keywords to bring up the desired content they need.
% Because of this, when interacting with the code generation model, the input query may not be concise enough, or ``natural'' enough to generate the desired code snippet.

% To this end, we need to separate the factors from an imperfect natural language to code generation model, with the factors lying in the query formation itself.
% We use an expert human Python programmer to act as an ``oracle'' code generation model.
% We give the human expert the query that the user issued and ask the expert to right the corresponding code snippet implementing the given input.
% If the expert could successfully output such code, then the query is good enough on its own by providing enough information to generate correct code, given a perfect code generation model.
% However, when developers issue queries, they implicitly have prior knowledge in their mind about the current code context they are working on, thus eliminating some information.
% A common example is the elimination of variable names defined in the previous contexts of the code that needs to be referenced during the intent being queried, or the omission of different types of flags and arguments that need to be supplied to the queried operation. 
% To fix this, we also provide the context code, which is the whole source code file snapshot at the time the query was issued, to the human expert, if the first attempt to generate code with just natural language queries failed.
% Note that the current state-of-the-art code generation model we use does not incorporate contextual information from current source code the developer is working on, and this analysis could provide insights on how to improve existing models.

% \gn{Could you give an example of ``good on its own'' and ``good with context'' in a table or something? I feel this explanation is a bit abstract.}

% Due to the limitation of human expert analysis costs, we randomly sampled 50 queries out of all queries issued during the user study, and ask human experts to attempt to generate code based on them.
% We record the success of generating code from queries without context and with context, representing cases of ``good'' formation of queries, and compare them with the data on what types of the candidates the developer eventually choose.
% We calculate the correlation between the human expert successes with code generation successes to investigate if code generation models require good and complete formation of queries with all the information needed.
% On the other hand, we look forward to investigate if retrieval methods are more robust to incomplete queries, or simply the concatenation of general keywords.
% Furthermore, we compare the percentage of the human expert successes among the sampled queries, using and not using the context, and see how much improvement would come from the current code context as supplementary information.

% \subsubsection{Results}
% Out of the sampled 50 queries, 38\% end up being selected by the user with the code generation candidate.
% 40\% of the queries are deemed ``good on its own'' following the manual query analysis procedure, and 68\% of the queries are deemed ``good with context''.
% Note that here ``good with context'' also includes all queries that are ``good on its own''.
% This is expected as code generation is not perfect and cannot handle all the well-defined queries, and it is also expected that some queries issued by the user are implicitly ignoring key information in the current code context at the time, as the user are assuming them.
% Without the context information, the query is usually under-specified and thus the code generation model would not perform as well.
% Looking at the percentage of the ``good queries'', we find that one outstanding barrier for deploying such code generation systems into real world development is that the user are not very often issue good queries that contain enough information even for a human programmer to implement the query intent.
% It is also the case that users sometime ignore to include key information inside the code context, like variables, etc. to inform the code generation model.
% This lead to potential gains in code generation model performance by incorporating more contextual information with natural language queries as input.

% Furthermore, we look at the correlation between the individual queries that are ``good on its own'' or ``good with context'', and those result in successful code generations.
% The Phi coefficient between whether the queries are ``good on its own'' and  whether the queries end up producing successful code generation results is 0.370 (p<0.05), suggesting moderate positive relationship.
% The Phi coefficient between whether the queries are ``good with context'' and whether the queries end up producing successful code generation results is 0.449 (p<0.05), suggesting strong positive relationship.
% From the positive correlation, we conclude that better query formulation is very crucial to the success of the code generation performance.



% \subsubsection{Approach}
% Since the current approaches for both code generation and code retrieval are far from perfect, users usually still need to go through the best candidate code snippet and make modifications to make them appropriate for the user intent within the current program context.

% Thus, we also analyze the amount of edits required for both code generation candidates and code retrieval edits.
% From our collected data, we can extract pairs selected code snippet candidates from the plugin, and the final modified code the user uploads.
% The user is asked to upload the code after the desired query is fulfilled in the code snippet after editing.

% To measure the extent of edits on the candidates, we adopt token-level edit distance, or Levenshtein distance.
% We first tokenize both the candidate code snippet and the final modified code snippet using Python tokenizer, and then calculate the edit distance based on two lists of tokens.
% This distance measures the number of token edits required for the developer to modify from generated/retrieved code to correct code inside the current context.
% We then compare the two distributions of edit distance for code generation and retrieval candidates statistically to investigate any properties.

% \subsubsection{Results}

% We analyze a total of 303 queries over all tasks in the user study that result in either generated or retrieved code candidates selected, inserted, edited to working code and then uploaded back to our server.
% From Figure~\ref{fig:edit_comparison}, we can see that overall code retrieval provides longer code snippet candidates that are selected by the user than code generation.
% After the user edits the code snippet, the length of code snippet that originates from code retrieval are also longer than that from code generation.
% As a result, it is expected that the retrieved code requires more edits to correct the code to suit the current programming code context, than those generated, as seen in Figure~\ref{fig:edit_comparison}.


% Furthermore, we are also interested in what kind of tokens tend to get modified from candidates to the final code snippet in the source code file.
% We count the frequency of tokens in both the original code snippets as well as the final edited code snippets, and normalize the frequency based on total token count in each corpus.
% We then compare what tokens' frequency increases and what tokens' frequency decreases the most, as shown in Table~\ref{tab:top-token-edits}.
% We find that the users are more likely to add common keywords like ``in, for, if, with'', builtin names and functions like ``key, print'' and common variable names like ``line, filename'' to the generated/retrieved candidates.
% This suggests that some code snippets are not perfect and users may still need to implement the desired functionality based on the existing baseline.
% Users are more likely to delete number and string literals from the code snippet, which is expected as many retrieved code snippets may be written for other scenarios that uses different literals, or uses hard-coded numbers as an example showcase.
% We also find some commonly used variable names like ``df, plt'' getting deleted, suggesting that variable replacement is one of the common operations when reusing the code snippets.
% An interesting observation here is that ``In'' and ``Out'' are getting deleted frequently, and we find that it's mostly due to some retrieved code snippets being shown in the format of IPython REPL, which uses ``In'' and ``Out'' to separate the Python source code and execution outputs.
% When integrating these snippets, the users will have to remove this excessive text.
% An example showcasing the user edits after selecting the candidate snippet is that the following:
% \begin{lstlisting}[frame=single,style=pythoncode]
% In [479]: df
% Out[479]: 
%     ID  birthyear   weight
% 0   619040  1962    0.123123
% 1   600161  1963    0.981742
% 2   25602033    1963    1.312312
% 3   624870  1987    0.942120

% In [480]: df["weight"].mean()
% Out[480]: 0.83982437500000007
% \end{lstlisting}
% gets edited to:
% \begin{lstlisting}[frame=single,style=pythoncode]
% car_prices = car_prices["price"].mean()
% \end{lstlisting}
% which involves deleting IPython REPL contents, as well as variable replacement and addition, as well as literal replacements.



% \begin{quote}
% ``I think sometimes the plugin can be intimidating, I feel like it is hard to get a complicated solution using it without more context. Perhaps sometimes when providing solutions from Stack Overflow, it could also provide a link to the solutions page? This may help the user with finding a more tailored solution for their program'' \partic{20}
% \end{quote}

% The plugin should show documentation and other accompanying context to educate the users more about the candidate code snippets.
% Participants state:
% \begin{quote}
% ``it would be really useful if the documentation ... otherwise it can be difficult to decide which of the suggestions is the correct one when you are not familiar with a module''. \partic{11}
% \end{quote}

% \paragraph{The plugin is situational} Participants think that the plugin is helpful in some areas more than others, especially that data analysis or machine learning related tasks are the worst where the plugin is performing, stating: 
% \begin{quote}
% ``for those easy tasks, like walk through the directory in filesystem, this plugin save my time because what i did previously is to go to stackoverflow can copy the code. But for difficult task like data processing or ML, the plugin is not helpful. Most snippet are not useful and i have to go to website like sklearn to read the full doc to understand what i should do'' \partic{3}
% \end{quote}
% \begin{quote}
% ``for working with both pandas and sklearn, the generated snippets made little sense and were not very relevant to what I requested.'' \partic{10}
% \end{quote}


% If the plugin could follow-up after initial query and ask the user to clarify their intents, or dissemble the complex functionality into smaller steps if the query is overall too high-level and general, then it could potentially be a better way of interacting, as participants state: 



% \begin{quote}
% ``... help find a more tailored solution would be if there could be some kind of chatbot functionality? What I mean by this is perhaps if you could identify the rough area in which the user needs assistance, a chatbot could help narrow it down further, helping to pinpoint an exact solution.'' \partic{20}
% \end{quote}
% This is also backed by some complaints on the way code generation expects queries to have variables, etc. are unnatural to developers, as they are used to only use keywords to search in web, stating: 
% \begin{quote}
% ``I am trying to incorporate variable names or strings when ask a question, however, most of the time, this variable name or string is not included in the tranX generated result. On the other hand, it is not very natural for me to `instantiate' my questions, I mostly like to search keywords or just a description of what I want to achieve.'' \partic{2}
% \end{quote}




% Next, we ask the question: How does the incorporation of a code generation and retrieval interface into the developer pipeline affect subjective user experience?
% For this research question, we perform qualitative and quantitative analysis based on the post-study user surveys described in Section~\ref{sec:postsurvey} \gn{Missing}.
% , we collect users' subjective evaluations post-task and post-study, about the user experience using the proposed hybrid approach of intelligent code generation.

% For the Likert scale based questions, we visualize the distribution to analyze how users think the plugin affects their development experience.
% For questions like ``What do you think worked well, compared with your previous ways to solve problems during programming?'' and ``What do you think should be improved, compared with your previous ways to solve problems during programming?'', we use \emph{card sorting}~\cite{Ritchie2013QualitativeRP} to qualitatively analyze the responses.
% Specifically, we go through all the responses received and cluster them into different aspects of what the users think.
% To do this, when going through all the responses, we segment each response into one or more key points, and put the point into an existing cluster if the point is similar in ideas to the points in that cluster, and put the point into a new cluster otherwise.
% Using this technique, we can generalize and categorize the current status of code generation and retrieval used in development, as well as the gaps to the ideal model, and the users' future expectations.

% \subsection{Results}
% \fx{add ref to participants, tracebility}

% We received a total of 38 post-study survey responses from the participants that completed all of the assigned tasks.
% We analyze the responses on their experience with the plugin as well as the task design.


% \subsubsection{Overall Plugin User Experience}
% We analyze users' reactions to the plugin experience.
% When asked the Likert-style question ``Overall, how was your experience using this plugin?'', the response statistics is shown in Figure~\ref{fig:survey_scores_overall}.
% We find that the responses are 54\% positive, 39\% neutral, and 5\% negative.
% This suggests that the plugin provides a good user experience for a majority of the participants.
% , and thus such intelligent programming interface embedded inside development environments should be promising.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/survey/survey_scores.pdf}
%     \caption{Overall experience of participants on using the plugin, ranging from 1 - very bad to 5 - very good.}
%     \label{fig:survey_scores_overall}
% \end{figure}

% \subsubsection{Advantages of Using the Plugin}
% \label{sec:subjective:advantages}
% For this purpose, we asked ``what do you think worked well, compared with your previous ways to solve problems during programming?'' for responses on the advantages of using the plugin.
% They can be categorized into the following:


% \paragraph{The plugin is useful for picking up those quick lines of code which the developer is aware of but cannot fully remember} Participants state:
% \begin{quote}
%     ``... particularly when all I need is one quick line of code or to remember the command for something'' \partic{20}
% \end{quote}
% \begin{quote}
%     ``on a few occasions, the plugin very conveniently gave me the snippet of code I was looking for. This was generally when the method was "on the tip of my tongue". Even just having the snippets mined from Stack Overflow visible in the IDE was a good memory refresher / source of ideas'' \partic{10}
% \end{quote}
% \begin{quote}
%     ``sometimes I just cannot remember the exact code, but I remember the shape. I could select the correct one easily'' \partic{2}
% \end{quote}
% \begin{quote}
%     ``it's really satisfying when it works; I could definitely see this being great in a later iteration. I enjoyed trying it out.'' \partic{10}
% \end{quote}

% \paragraph{In-IDE plugin is less disruptive than using web browser}
% Participants state that ``the plugin stops me having to go and search online for solutions, particularly when all I need is one quick line of code or to remember the command for something, ..., it can be very easy to get distracted when searching for solutions online, so I feel like the plugin is something which would help improve my overall efficiency'', ``having an integrated method to suggest code snippets is very handy, especially for API usages. Compared with manual search, this is faster and less disruptive.''

% \paragraph{The effect of the plugin may be particularly important for languages requiring a lot of library usages like Python}
% Participants state:
% \begin{quote}
% ``Python is an easy language due to the huge number of supported libraries that's why it also needs a lot of searching in the behavior and syntax and this was the benefit of the plugin.'' \partic{21}
% \end{quote}

% \paragraph{The plugin is situational} Participants think that the plugin is helpful in some areas more than others, especially that data analysis or machine learning related tasks are the worst where the plugin is performing, stating: 
% \begin{quote}
% ``for those easy tasks, like walk through the directory in filesystem, this plugin save my time because what i did previously is to go to stackoverflow can copy the code. But for difficult task like data processing or ML, the plugin is not helpful. Most snippet are not useful and i have to go to website like sklearn to read the full doc to understand what i should do'' \partic{3}
% \end{quote}
% \begin{quote}
% ``for working with both pandas and sklearn, the generated snippets made little sense and were not very relevant to what I requested.'' \partic{10}
% \end{quote}

% \paragraph{Using the plugin will require some knowledge and practice} Participants state:
% \begin{quote}
% ``... useful to me towards the end when I got the hang of it and could formulate questions in the correct way to it (which I feel, qualifies is somewhat of a skill in itself - for this version of the plugin)'' \partic{15}
% \end{quote}
% \begin{quote}
% ``the plugin excels in letting you look up little syntax bits that you have forgotten, but where you have a good background understanding of the underlying principles/modules/frameworks.'' \partic{11}
% \end{quote}
% \begin{quote}
% ``for more complex problem, I think that the plugin does not help at all, because the programmer need to know the theoretical background.'' \partic{16}
% \end{quote}

% \subsubsection{Disadvantages of the Plugin and Possible Improvements}
% \label{sec:subjective:improvements}
% For this purpose, we asked ``What do you think should be improved, compared with your previous ways to solve problems during programming?'' and ``Do you have any other suggestions/comments for the plugin?''
% The responses can be categorized as:

% \paragraph{More context should be shown} Participants think that contexts including explanations, documentations should be included alongside the generated code so that the user could understand what the snippet is supposed to do if the user does not have enough previous knowledge, stating:
% \begin{quote}
% ``I think sometimes the plugin can be intimidating, I feel like it is hard to get a complicated solution using it without more context. Perhaps sometimes when providing solutions from Stack Overflow, it could also provide a link to the solutions page? This may help the user with finding a more tailored solution for their program'' \partic{20}
% \end{quote}
% \begin{quote}
% ``I hope the code snippet generated can have more comments or usage. Otherwise I still need to search web to understand what it is.'' \partic{3}
% \end{quote}

% The plugin should show documentation and other accompanying context to educate the users more about the candidate code snippets.
% Participants state:
% \begin{quote}
% ``it would be nice if the examples from the internet could contain the relevant context of the discussion (e.g., things to consider when using this suggestion), as well as the input/output examples.'' \partic{5}
% \end{quote}
% \begin{quote}
% ``it would be really useful if the documentation ... otherwise it can be difficult to decide which of the suggestions is the correct one when you are not familiar with a module''. \partic{11}
% \end{quote}


% \paragraph{Code generation and retrieval result quality should be further improved} Some participants are not satisfied with the quality of both code generation and code retrieval, but even if the plugin is not showing perfect code, it serves as a good reference. 
% Participants state:
% \begin{quote}
% ``it was rare when i can use a code from plugin in a straight way but it's still cool to watch some examples.'' \partic{7}
% \end{quote}
% \begin{quote}
% ``the SOTA model needs some improvements.'' \partic{4} 
% \end{quote}
% \begin{quote}
% ``results of the plugin sometime is not related to the search.'' \partic{14}
% \end{quote}
% \begin{quote}
% ``sometimes i don't find what i'm searching for.'' \partic{31}
% \end{quote}


% \paragraph{Better interactive form}
% If the plugin could follow-up after initial query and ask the user to clarify their intents, or dissemble the complex functionality into smaller steps if the query is overall too high-level and general, then it could potentially be a better way of interacting, as participants state: 
% \begin{quote}
% ``... help find a more tailored solution would be if there could be some kind of chatbot functionality? What I mean by this is perhaps if you could identify the rough area in which the user needs assistance, a chatbot could help narrow it down further, helping to pinpoint an exact solution.'' \partic{20}
% \end{quote}
% This is also backed by some complaints on the way code generation expects queries to have variables, etc. are unnatural to developers, as they are used to only use keywords to search in web, stating: 
% \begin{quote}
% ``I am trying to incorporate variable names or strings when ask a question, however, most of the time, this variable name or string is not included in the tranX generated result. On the other hand, it is not very natural for me to `instantiate' my questions, I mostly like to search keywords or just a description of what I want to achieve.'' \partic{2}
% \end{quote}

% \paragraph{Retrieved code has too much scaffold}
% Participants noted that the retrieved code snippets usually contain a lot of content that set up the environment, but the user may only need the core line in it, and thus wasting a lot of time only to extract the needed part out of it, stating:
% \begin{quote}
% ``sometimes I want to generate an expression to be inserted somewhere, to be assigned to a variable, or to match the indentation level, without having to tell the plugin this explicitly. I didn't feel like the plugin was aware of context.'' \partic{10}
% \end{quote}

% \subsubsection{Task Design and Assignment Suitability}
% \label{sec:subjective:taskdesign}
% We asked ``What did you think of the tasks assigned to you in general?'' during the post-study survey.
% The utility of these questions is demonstrating that the tasks are useful, and that the tasks used in the study provide a good test bed for future research as well.
% The responses can be categorized into several themes:

% \paragraph{Tasks are easy and comfortable to deal with} Participants state: 
% \begin{quote}
% ``the tasks were different and interesting.'' \partic{22}
% \end{quote}
% \begin{quote}
% ``... think that most of the task was easy and 1 or 2 task between the easy and intermediate.'' \partic{29}
% \end{quote}

% \paragraph{Tasks are of varied difficulty} Participants claim that some tasks are challenging to them but all of them are covering different areas in Python overall, stating: 
% \begin{quote}
% ``I thought the tasks were interesting and fun and offered variety, which helped me learn new things.'' \partic{13}
% \end{quote}
% \begin{quote}
% ``I think that the task were quite challenging but they correct evaluate the capacity of the candidate, as well as the impact of using the plugin functionality''
% \partic{16}
% \end{quote}
% \begin{quote}
% ``Address several coding/programming skills, vary in degree of hardness, I enjoyed them.''\partic{17}
% \end{quote}


% \paragraph{Tasks are suitable for testing scenarios that requires a lot of searching} Participants state:
% \begin{quote}
% ``... requires fairly amount of search. Some of them are very tricky.'' \partic{4}
% \end{quote}
% \begin{quote}
% ``they seemed to be chosen in a manner such that a person who is not in constant practice of a library would have to search for the API docs online or ask the plugin a question.'' \partic{15}
% \end{quote}
% \begin{quote}
% ``I think the tasks had an appropriate mixture of difficulties to test impact of the plug-in.'' \partic{11}
% \end{quote}

